Long-Period Transients as a new frontier in time-domain astronomy

Long-period radio transients (LPTs) are relatively new astrophysical objects occupying the observational gap between canonical pulsars and slowly varying radio variables. They emit coherent, highly polarised radio bursts with periods from minutes to hours, often exhibiting millisecond- to minute-scale substructure, short duty cycles, and broadband emission. Their radio luminosities typically exceed what rotational energy alone can power, necessitating alternative energy sources such as magnetic field decay, magnetospheric reconnection, or binary interactions. As multiwavelength counterparts in X-ray, optical, and infrared bands provide key constraints on progenitors and emission mechanisms, observational evidence points to a diverse progenitor population including ultra-long period magnetars and magnetic white dwarf binaries. Fast imaging surveys with SKAO and its precursors are opening a new discovery space, enabling systematic detection, high-cadence monitoring, and detailed follow-up. Despite the challenges of high extinction, intermittent emission, and computational demands for discovery, the expanding LPT population provides a new laboratory for studying coherent radio emission in a range of compact-object systems, from pulsars to white dwarf binaries. This diversity allows us to test how the emission processes depend on magnetic field strength, rotation, and binary interaction.

==> individual_sources.tex <==
\subsection{Polarization} 
\td{Coordinating authors to shorten this section}
\begin{itemize}
\item \textbf{GPM J1839-10} [\citep{hurley2023long}][\citep{men2025highly}]\\
GPM J1839$-$10 exhibits polarization properties dominated by linear polarization, 
with significant though variable circular polarization, long-term stability of its rotation 
and dispersion measures (RM/DM), unusual polarization conversion phenomena, 
and the presence of polarized substructures.  

The linear polarization fraction spans an exceptionally broad range, from $\sim$10\% up to nearly 100\%. 
The polarization angle (PA) is generally flat, but some pulses show abrupt $\pm 90^{\circ}$ jumps, 
closely resembling the orthogonal polarization modes (OPMs) commonly observed in pulsars.  

The circular polarization fraction is typically low but significant, 
remaining $<$10\% for most pulses but reaching peaks as high as 95\% in specific pulse phases or substructures. 
A notable feature is the correlation between CP sign reversals and rapid PA swings: 
when the PA exhibits steep variations, the CP sign often flips. 
This behavior is consistent with the polarization characteristics of normal pulsars 
and radio magnetars (e.g., XTE~J1810$-$197), and is generally interpreted as a geometric effect 
arising when the line of sight traverses the emission cone within the magnetosphere.  

The RM and DM of J1839$-$10 remain stable over long timescales, 
indicating that the observed polarization properties are intrinsic to the source rather than arising from interstellar propagation effects.  

High-resolution MeerKAT observations in 2023 revealed unusual polarization conversion phenomena, 
including both frequency-dependent linear-to-circular conversion and down-drifting polarization conversion. 
In the first case, linear and circular polarization fractions display complementary frequency dependence: 
linear polarization dominates at lower frequencies, while the circular fraction increases at higher frequencies. 
In the second case, a drifting polarization-conversion band was detected: 
within this band, the CP fraction rises from $<$10\% to $>$50\% while the LP fraction decreases correspondingly, 
and the total intensity drops by $\sim$50\%. 
These effects cannot be attributed to calibration errors or interstellar medium propagation. 
As the first reported case of a combined polarization-conversion and frequency-drifting phenomenon in an LPT, 
this behavior may indicate dynamically evolving flux tubes or plasma clumps in the source region.  

Moreover, the polarized substructures, downward frequency-drifting features, 
and frequency-dependent evolution of the polarization vector observed in GPM J1839$-$10 
closely resemble those of repeating fast radio bursts (FRBs), such as FRB~20121102A and FRB~20201124A, 
providing further evidence of a possible physical connection.  

Although the polarization properties of J1839$-$10 suggest a pulsar or magnetar origin, 
the unified geometric model proposed by Horváth et al.~\citep{horvath2025unified} 
argues that this LPT may instead be consistent with a white dwarf binary pulsar system.  

\item \textbf{GLEAM-X J162759.5-523504.3}[\citep{hurley2022radio}]\\
GLEAM-X~J1627$-$5235 exhibits strong and persistent linear polarization, with a polarization fraction of up to 88\%, but shows no evidence for significant circular polarization. 
This lack of circularly polarized emission suggests that the source is unlikely to belong to populations typically dominated by circular polarization, such as flare stars, exoplanetary interactions, or white dwarf/M-dwarf binaries.  

The polarization angle remains stable across both pulse phase (within individual pulses) 
and observation time (over several months), consistent with a steady and well-ordered magnetic field geometry. 
A pulse-phase-resolved rotation measure (RM) analysis further demonstrates that the RM is constant 
even within individual pulses, thereby ruling out transient Faraday rotation effects, 
such as plasma turbulence in the immediate source environment.  

\item \textbf{ASKAP J1935+2148}[\citep{caleb2024emission}]\\
ASKAP~J1935+2148 exhibits polarization properties that are closely tied to its three distinct emission states, 
with critical differences in polarization type (linear vs.\ circular), fraction, and stability. 
These states are summarized in Table~\ref{tab:emission_states}.  

\begin{table*}[ht]
\centering
\begin{tabularx}{\textwidth}{l l X X X}
\toprule
\textbf{Emission State} & \textbf{Telescope} & \textbf{Polarization Dominance} & \textbf{RM ($\mathrm{rad\,m^{-2}}$)} & \textbf{PA} \\
\midrule
Strong Pulse Mode & ASKAP &
  \makecell[tl]{Linear (Q/U) \\ $>$90\% linear; \\$<$3\% circular} &
  $+159.3\pm0.3$ &
  Flat (no variation with pulse phase or observation time) \\
Weak Pulse Mode & MeerKAT &
  \makecell[tl]{Circular (V) \\ $\sim$40\% linear; \\$>$70\% circular} &
  $+159.1\pm0.3$ &
  Flat (measurable only in high-S/N detections) \\

Quiescent Mode & \makecell[tl]{ASKAP\\MeerKAT} &
  No detectable polarization &
  N/A & N/A \\
\bottomrule
\end{tabularx}
\caption{Polarization properties of the three emission states of ASKAP~J1935+2148.}
\label{tab:emission_states}
\end{table*}

In both the strong and weak modes, J1935+2148 exhibits a stable rotation measure (RM). 
Comparison with the RMs of nearby pulsars, obtained from the ATNF Pulsar Catalogue, confirms that the measured RM originates in the Galactic interstellar medium (ISM), with no evidence for additional, locally imparted Faraday rotation.  

In summary, the state-dependent polarization of ASKAP~J1935+2148—dominated by high linear polarization in the strong mode and by strong circular polarization in the weak mode—distinguishes it from other known long-period transients. 
These polarization characteristics strongly support an origin in an ultralong-period magnetar or neutron star.  

% \item \textbf{ILT J1101+5521} [\cite{de2025sporadic}]\\
% The polarization properties of J1101+5521 exhibit pulse-to-pulse variability. 
% The peak linear polarization fraction ranges from approximately 51\% to 13\%, with no significant circular polarization detected. 
% Rotation measures (RMs) derived from individual pulses remain consistent, 
% indicating no measurable local contribution from the stellar corona or wind of the system.  

% Although J1101+5521 is within a white dwarf binary system,  the high degree of linear polarization is indicative of strongly ordered magnetic fields,  as expected for white dwarfs. 
% Conversely, the absence of significant circular polarization is inconsistent with the typical  low-frequency radio emission observed from M dwarfs, which generally exhibit strong circular 
% polarization (often exceeding 38\%, even in relatively weak sources). 
% These characteristics therefore support the interpretation that the radio emission originates from the white dwarf itself, or from interactions between the white dwarf and its M-dwarf companion. 

\item \textbf{ASKAP/DART J1832$-$0911} [\cite{li202444,wang2025detection}]\\
LPT~J1832$-$0911 exhibits both linear polarization (LP) and circular polarization (CP), with their occurrence and intensity strongly dependent on the source’s emission state (active vs. quiescent) and pulse mode (wide vs. narrow). 

The polarization properties are geometrically stable across observing epochs. CP components are detected exclusively in the wide-pulse mode (pulse width: 100--300~s) during the active emission state, and are confined to the trailing edge of the pulse, as shown in Fig.\ref{J1832-0911}. In contrast, no CP is observed in the narrow-pulse mode (pulse width: $\sim$40~s). 


\begin{figure}[h]
    \centering
	\includegraphics[width=0.48\columnwidth]{Figures/J1832_1.png}
    \includegraphics[width=0.48\columnwidth]{Figures/J1832_2.png}
    \caption{The phase-locked circular polarization of J1832-0911 at different emission states (left panel: Di Li et al. 2024; Right panel: Ziteng W et al. 2025).}
    \label{J1832-0911}
\end{figure}

The CP components are phase-locked, occurring at fixed pulse phases, and are temporally narrow, spanning less than 3\% of the rotation period. This behavior suggests that circularly polarized emission originates from a confined region of the magnetosphere. 

Furthermore, most CP components exhibit sign reversals. Such reversals are plausibly caused by the line of sight sweeping across the minimum angle between the observer’s view and the magnetic axis of the source, consistent with geometric interpretations of pulsar and magnetar polarization. 


\item \textbf{CHIME/ILT J1634+44}[\cite{dong2025chime,bloot2025strongly}]\\
The polarization properties of J1634+44 are highly unusual. All detected radio pulses from J1634+44 exhibit a total polarization fraction (sum of circular and linear components) of ~100\%, indicating the emission is intrinsically coherent (incoherent mechanisms cannot produce such high polarization).

This LPT switches between two distinct polarization states on a pulse-to-pulse basis. (1) Fully circularly polarized (CP) pulses: Detected in both Stokes V observations (CHIME, VLA, LOFAR). The VLA measured a lower limit of 98\% CP, and CHIME data confirmed |V|/I >= 0.9. The circular polarization is intrinsic (not caused by propagation effects like Faraday conversion), as it remains stable across a decade of observing frequencies (400 MHz-1.4 GHz).
(2) Fully linearly polarized (LP) pulses: Observed in LOFAR data, with |L|/I >= 0.89. One pulse even reached ~98\% linear polarization. CHIME data also noted non-negligible intrinsic linear polarization in some bursts.

The reported observation confirmed that the high polarization fraction (either CP or LP) is stable across frequencies, ruling out propagation-induced polarization changes (e.g., Faraday rotation).

Additionally, the polarization of this source is phase dependent, shown in Fig.\ref{iltJ1634}. The research claims that the detectable pulses only arriving after two or three rotations with a speccific period at 841 s.  Bloot et al. (2025) found a clear link between polarization state and pulse timing:
Pulses arriving after 2 rotations of the 841 s period are almost always fully circularly polarized.
Pulses arriving after 3 rotations are mostly fully linearly polarized (only one exception).
\begin{figure}[h]
    \centering
	\includegraphics[width=0.9\columnwidth]{Figures/ILT1634.png}
    \caption{Phase-dependent switching between circular and linear polarization (Bloot et al. 2025).}
    \label{iltJ1634}
\end{figure}

The extreme polarization (100\% CP/LP) and its stability imply the emission mechanism is pulsar-like (Dong et al. 2025) or driven by relativistic electron-cyclotron maser instability (ECMI) (Bloot et al. 2025).

\item \textbf{ASKAP J144834$-$685644} [\cite{anumarlapudi2025askap}]\\
ASKAP~J1448$-$6856 exhibits a steep radio spectrum and a spectral energy distribution (SED) peaking in the near-ultraviolet, consistent with a hot, strongly magnetized source. 

Its polarization properties are extreme and highly variable. Individual bursts show strong polarization (35--100\%), most often elliptical. Episodes of nearly 100\% circular polarization are observed, although the emission is never purely linear. Polarization varies both between epochs and within single bursts, including circular polarization sign reversals (flips) and, in some cases, the appearance of a circularly polarized interpulse.  

A particularly distinctive property of this LPT is its cut-off and narrow-band emission structure. For instance, an ATCA burst observed on 2024 July 15 (1.1--3.1~GHz) vanished completely above $\sim$1.5~GHz. Below this cut-off, the polarized emission was confined to discrete, narrow frequency bands, rather than forming a continuous spectrum. This behavior is consistent with ASKAP (799--1090~MHz) and MeerKAT observations. Polarization also exhibits strong frequency dependence: in the UHF band (544--1088~MHz), bursts are elliptically polarized with comparable linear and circular contributions, while in the L-band (856--1712~MHz), circular polarization dominates (often $>$80\%) and linear polarization is strongly suppressed. At these higher frequencies, the narrow-band clustering becomes more pronounced, with bandwidths below 10~MHz in some bursts.  

These properties strongly support a coherent emission process in a magnetized plasma, most plausibly electron cyclotron maser emission or a magnetar-like mechanism. The combination of a steep spectrum, strong and variable polarization, circular sign reversals, and frequency-dependent narrow-band structure clearly distinguishes ASKAP~J1448$-$6856 from ordinary pulsars, instead pointing to a connection with magnetars or magnetic white-dwarf binaries.

\item \textbf{ASKAP J175534.9$-$252749.1} [\cite{Dobie2024}]\\
ASKAP~J175534.9$-$252749.1 (hereafter J1755$-$2527) exhibits distinct polarization characteristics that are both constrained by observational limitations and informative about the source's physical properties.

Polarized emission from J1755$-$2527 is not detected uniformly across all observations; it is observed only in specific telescopes, frequency bands, and high signal-to-noise (S/N) pulses. In particular, polarization was confirmed in just three sufficiently bright pulses, all recorded by telescopes with higher sensitivity or optimal beam centering.  

(1) No significant linear or circular polarization was detected in Murchison Wide-field Array (MWA) observations at 154--215~MHz, even after optimizing the frequency resolution (10~kHz) to reduce Faraday depolarization. This non-detection is likely due to MWA’s relatively high noise floor ($\sim$80~mJy~beam$^{-1}$ at 4~s time resolution) and potential depolarization caused by interstellar Faraday rotation.  

(2) Similarly, ATCA observations in the L- and S-bands (1.1--3.1~GHz) did not reveal polarized emission, likely because the pulses were faint (4--5$\sigma$ detections) and exhibited strong pulse-to-pulse variability.  

The three polarized pulses that were detected display consistent rotation measure (RM) magnitudes over the 2023--2024 period. This stability indicates that there were no significant changes in the interstellar medium (ISM) along the line of sight, nor in the intrinsic magnetic field of the source, over the one-year observation window.


\end{itemize}

==> journal-names.tex <==
\newcommand{\actaa}{Acta Astron.} % Acta Astronomica
\newcommand{\araa}{ARA\&A} % Annual Review of Astron and Astrophys
\newcommand{\aar}{A\&ARv} % Astrononmy \& Astrophysics Review
\newcommand{\aapr}{A\&ARv} % Astronomy\&Astrophysics Reviews
\newcommand{\ab}{Astrobiol.} % Astrobiology
\newcommand{\aj}{AJ} % Astronomical Journal
\newcommand{\apj}{ApJ} % Astrophysical Journal
\newcommand{\apjl}{ApJL} % Astrophysical Journal, Letters
\newcommand{\apjs}{ApJSS} % Astrophysical Journal, Supplement
\newcommand{\ao}{Appl. Opt.} % Applied Optics
\newcommand{\apss}{Astro. \& Space Sci.} % Astrophysics and Space Science
\newcommand{\aap}{A\&A} % Astronomy and Astrophysics
\newcommand{\aaps}{A\&AS.} % Astronomy and Astrophysics, Supplement
\newcommand{\baas}{Bull. Am. Astron. Soc.} % Bulletin of the AAS
\newcommand{\caa}{Chinese A\&A} % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{Chinese J. A\&A} % Chinese Journal of Astronomy and Astrophysics
\newcommand{\cqg}{Class. Quantum Gravity} % Classical and Quantum Gravity
\newcommand{\gal}{Galaxies} % Galaxies
\newcommand{\gca}{Geo. Cosmo. Acta} % Geochimica Cosmochimica Acta
\newcommand{\icarus}{Icarus} % Icarus
\newcommand{\jcap}{JCAP} % Journal of Cosmology and Astroparticle Physics
\newcommand{\jgr}{J. Geophys. Res.} % Journal of Geophysics Research
\newcommand{\jgrp}{J. Geophys. Res. Planets} % Journal of Geophysics Research: Planets
\newcommand{\jqsrt}{J. Quant. Spectrosc. Radiat. Transf.} % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand{\memsai}{Mem. SAIt} % Mem. Societa Astronomica Italiana
\newcommand{\mnras}{MNRAS} % Monthly Notices of the RAS
\newcommand{\nat}{Nature} % Nature
\newcommand{\nastro}{Nat. Astron.} % Nature Astronomy
\newcommand{\ncomms}{Nat. Commun.} % Nature Communications
\newcommand{\nphys}{Nat. Phys.} % Nature Physics
\newcommand{\na}{New Astron.} % New Astronomy
\newcommand{\nar}{New Astron. Rev.} % New Astronomy Review
\newcommand{\physrep}{Phys. Rep.} % Physics Reports
\newcommand{\pra}{Phys. Rev. A} % Physical Review A: General Physics
\newcommand{\prb}{Phys. Rev. B} % Physical Review B: Solid State
\newcommand{\prc}{Phys. Rev. C} % Physical Review C
\newcommand{\prd}{Phys. Rev. D} % Physical Review D
\newcommand{\pre}{Phys. Rev. E} % Physical Review E
\newcommand{\prx}{Phys. Rev. X} % Physical Review X
\newcommand{\prl}{Phys. Rev. Let.} % Physical Review Letters
\newcommand{\psj}{Planet. Sci. J.} % Planetary Science Journal
\newcommand{\planss}{Planet. Space Sci.} % Planetary Space Science
\newcommand{\pnas}{Proc. Natl Acad. Sci. USA} % Proceedings of the US National Academy of Sciences
\newcommand{\procspie}{Proc. SPIE} % Proceedings of the SPIE
\newcommand{\pasa}{PASA} % Publications of the Astron.  Soc. of Australia
\newcommand{\pasj}{PASJ} % Publications of the Astron.  Soc. of Japan 
\newcommand{\pasp}{PASP} % Publications of the Astron.  Soc. of the Pacific
\newcommand{\rmxaa}{RMXAA} % Revista Mexicana de Astronomia y Astrofisica
\newcommand{\sci}{Science} % Science
\newcommand{\sciadv}{Sci. Adv.} % Science Advances
\newcommand{\solphys}{Sol. Phys.} % Solar Physics
\newcommand{\sovast}{Soviet Ast.} % Soviet Astronomy
\newcommand{\ssr}{Space Sci. Rev.} % Space Science Reviews
\newcommand{\uni}{Universe} % Universe

